Multiple Beamforming with Perfect Coding

Perfect Space-Time Block Codes (PSTBCs) achieve full diversity, full rate, nonvanishing constant minimum determinant, uniform average transmitted energy per antenna, and good shaping. However, the high decoding complexity is a critical issue for practice. When the Channel State Information (CSI) is available at both the transmitter and the receiver, Singular Value Decomposition (SVD) is commonly applied for a Multiple-Input Multiple-Output (MIMO) system to enhance the throughput or the performance. In this paper, two novel techniques, Perfect Coded Multiple Beamforming (PCMB) and Bit-Interleaved Coded Multiple Beamforming with Perfect Coding (BICMB-PC), are proposed, employing both PSTBCs and SVD with and without channel coding, respectively. With CSI at the transmitter (CSIT), the decoding complexity of PCMB is substantially reduced compared to a MIMO system employing PSTBC, providing a new prospect of CSIT. Especially, because of the special property of the generation matrices, PCMB provides much lower decoding complexity than the state-of-the-art SVD-based uncoded technique in dimensions 2 and 4. Similarly, the decoding complexity of BICMB-PC is much lower than the state-of-the-art SVD-based coded technique in these two dimensions, and the complexity gain is greater than the uncoded case. Moreover, these aforementioned complexity reductions are achieved with only negligible or modest loss in performance.

==> Generalization.tex <==
\section{Generalization to Larger Dimensions} \label{sec:Generalization}
\subsection{PCMB}
For PCMB of dimensions $3$, $4$, and $6$, it can be proved that they all achieve the full diversity order by analyzing the PEP in a similar way to Section \ref{sec:GCMB}-A.

Similarly to GCMB, the elements of $\mathbf{\Lambda X}$ for PCMB are related to only one of the $\mathbf{x}_v$, thus can be divided into $D$ groups. The received signal is then divided into $D$ parts, which can be represented as
\begin{align}
\mathbf{y}_v = \mathbf{\Phi}_v \mathbf{\Lambda G} \mathbf{x}_v + \mathbf{n}_v, 
\label{eq:eq:deteced_symbol_decomposed_pcmb}
\end{align} 
where $\mathbf{\Phi}_v=\textrm{diag}(\phi_{v,1}, \cdots, \phi_{v,D})$ is a diagonal unitary matrix whose elements satisfy
\begin{align*}
{\phi}_{v,k} = \left\lbrace 
\begin{array}{cc}
1, & 1 \leq k \leq D+1-v, \\
g, & D+2-v \leq k \leq D.
\end{array} \right.
\end{align*} 

By using the QR decomposition of $\mathbf{\Lambda G}=\mathbf{Q} \mathbf{R}$, and moving $\mathbf{\Phi}_v\mathbf{Q}$ to the left hand, (\ref{eq:eq:deteced_symbol_decomposed_pcmb}) is rewritten as 
\begin{align}
\tilde{\mathbf{y}}_v = \mathbf{Q}^H \mathbf{\Phi}_v^H \mathbf{y}_v = \mathbf{R}\mathbf{x}_v + \mathbf{Q}^H \mathbf{\Phi}_v^H \mathbf{n}_v = \mathbf{R}\mathbf{x}_v + \tilde{\mathbf{n}}_v.
\label{eq:deteced_symbol_decomposed_pcmb_2}
\end{align}

For the dimension of $4$, the $\mathbf{R}$ matrix in (\ref{eq:deteced_symbol_decomposed_pcmb_2}) is real-valued,  which can be proved in a similar way to that in Section \ref{sec:GCMB}-B. Consequently, the real part and the imaginary part of $\mathbf{x}_v$ can be decoded separately, in a similar way to GCMB. Real-valued SD with the last layer rounded can be employed to decode (\ref{eq:deteced_symbol_decomposed_pcmb_2}). The worst-case decoding complexity of PCMB is then $\mathcal{O}(M^{1.5})$. Regarding MIMO systems using PSTBC, the worst-case decoding complexity is $\mathcal{O}(M^{13.5})$ by using a similar decoding technique to \cite{Sinnokrot_FMLD_GC}, \cite{Sinnokrot_GC_FD}. For FPMB, ML decoding can be achieved by using SD based on the real lattice representation in \cite{Azzam_SD_NLR}, \cite{Azzam_SD_RLR}, plus quantization of the last two layers, and the worst-case complexity is $\mathcal{O}(M^{3})$.

For the $D=3$ dimension case, the $\mathbf{R}$ matrix is complex-valued. Therefore, the real and the imaginary parts of $\mathbf{x}_v$ cannot be decoded separately, unlike the case of $D=2,4$. Moreover, since the M-HEX constellation is used instead of M-QAM, a complex-valued SD is needed. The worst-case decoding complexity of PCMB is then $\mathcal{O}(M^{3})$. In the case of general MIMO systems using PSTBC, the worst-case decoding complexity is $\mathcal{O}(M^{9})$. For FPMB, the worst-case decoding complexity is $\mathcal{O}(M^{2})$.

In the case of $D=6$, which is similar to $D=3$, the $\mathbf{R}$ matrix is complex-valued, and M-HEX signals are transmitted. Consequently, the worst-case decoding complexity of PCMB is $\mathcal{O}(M^{6})$, while the worst-case decoding complexity of general MIMO systems using PSTBC and FPMB are $\mathcal{O}(M^{36})$ and $\mathcal{O}(M^{5})$ respectively.

\subsection{BICMB-PC}
For BICMB-PC of dimensions $3$, $4$, and $6$, a similar method to that in Section \ref{sec:BICMB-GC}-A analyzing the PEP can be applied to prove they all achieve the full diversity order.

Since the elements of $\mathbf{\Lambda} \mathbf{Z}_k$ for BICMB-PC are related to only one of the $\mathbf{x}_{v,k}$, which is similar to BICMB-GC, it can be divided into $D$ groups. Then the received signal, which is divided into $D$ parts, can be represented as
\begin{align}
\mathbf{\breve{y}}_{v,k} = \mathbf{\Phi}_v \mathbf{\Lambda G} \mathbf{x}_{v,k} + \mathbf{\breve{n}}_{v,k}.
\label{eq:deteced_symbol_decomposed_bicmb-pc}
\end{align} 

By using the QR decomposition of $\mathbf{\Lambda G}=\mathbf{Q} \mathbf{R}$, and moving $\mathbf{\Phi}_v\mathbf{Q}$ to the left hand, (\ref{eq:deteced_symbol_decomposed_bicmb-pc}) is rewritten as 
\begin{align}
\tilde{\mathbf{y}}_{v,k} = \mathbf{Q}^H \mathbf{\Phi}_v^H \mathbf{\breve{y}}_{v,k} = \mathbf{R}\mathbf{x}_{v,k} + \mathbf{Q}^H \mathbf{\Phi}_v^H \mathbf{\breve{n}}_{v,k} = \mathbf{R}\mathbf{x}_{v,k} + \tilde{\mathbf{n}}_{v,k}.
\label{eq:deteced_symbol_decomposed_bicmb-pc_2}
\end{align}
Then the ML bit metrics in (\ref{eq:ML_decoding_bicmb-pc}) can be simplified as (\ref{eq:ML_decoding_bicmb-pc_2}) in Section \ref{sec:BICMB-GC}-B.

In the case of $D=4$, the $\mathbf{R}$ matrix in (\ref{eq:deteced_symbol_decomposed_bicmb-pc_2}) is real-valued, which can be proved in a similar way to Section \ref{sec:GCMB}-B. As a result, the real and imaginary parts of $\mathbf{\tilde{y}}_{m,k}$ in (\ref{eq:ML_decoding_bicmb-pc_2}) can be separated, and only the part corresponding to the coded bit is required for calculating one bit metric of the Viterbi decoder. Assume that square $M$-QAM is used. Then, the ML bit metrics in (\ref{eq:ML_decoding_bicmb-pc_2}) can be further simplified as (\ref{eq:ML_bit_metrics_real}) if $c_{k'}$ is mapped to the real part, or (\ref{eq:ML_bit_metrics_imag}) if $c_{k'}$ is mapped to the imaginary part. Therefore, the worst-case complexity of calculating one bit metric is only $\mathcal{O}(M^{1.5})$ by using a real-valued SD with the last layer rounded. On the other hand, BICMB-FP has the worse-case complexity of $\mathcal{O}(M^{3})$ by using a real-valued SD based on the real lattice representation in \cite{Azzam_SD_NLR}, \cite{Azzam_SD_RLR}, plus quantization of the last two layers.

For the dimension of $3$, the $\mathbf{R}$ matrix is complex-valued. Therefore, the real and the imaginary parts of $\mathbf{\tilde{y}}_{m,k}$ cannot be separated, unlike the case of $D=2,4$. Moreover, since the M-HEX constellation is used instead of M-QAM, a complex-valued SD is needed. The worst-case complexity of BICMB-PC to derive one bit metric is then $\mathcal{O}(M^{3})$. For BICMB-FP, the worst-case complexity is $\mathcal{O}(M^{2})$.

For the $D=6$ dimension case, which is similar to $D=3$, the $\mathbf{R}$ matrix is complex-valued, and M-HEX signals are transmitted. As a result, the worst-case complexity of BICMB-PC is $\mathcal{O}(M^{6})$, while that of BICMB-FP is $\mathcal{O}(M^{5})$.
